Active Event Alignment for Monocular Distance Estimation

Event cameras provide a natural and data efficient representation of visual information, motivating novel computational strategies towards extracting visual information. Inspired by the biological vision system, we propose a behavior driven approach for object-wise distance estimation from event camera data. This behavior-driven method mimics how biological systems, like the human eye, stabilize their view based on object distance: distant objects require minimal compensatory rotation to stay in focus, while nearby objects demand greater adjustments to maintain alignment. This adaptive strategy leverages natural stabilization behaviors to estimate relative distances effectively. Unlike traditional vision algorithms that estimate depth across the entire image, our approach targets local depth estimation within a specific region of interest. By aligning events within a small region, we estimate the angular velocity required to stabilize the image motion. We demonstrate that, under certain assumptions, the compensatory rotational flow is inversely proportional to the object's distance. The proposed approach achieves new state-of-the-art accuracy in distance estimation - a performance gain of 16% on EVIMO2. EVIMO2 event sequences comprise complex camera motion and substantial variance in depth of static real world scenes.

==> figures/more_result_big.tex <==
\def\figWidth{0.2\linewidth}
% \def\figheit{height=1.2cm}
% \def\figsize{height=1.2cm, width=1.6cm}
\begin{figure*}
	\centering
    {\small
    \setlength{\tabcolsep}{0.5pt}
    
	\begin{tabular}{
	>{\centering\arraybackslash}m{0.195\linewidth} 
	>{\centering\arraybackslash}m{\figWidth}
	>{\centering\arraybackslash}m{\figWidth}
 	>{\centering\arraybackslash}m{\figWidth} 
	>{\centering\arraybackslash}m{\figWidth} 
	>{\centering\arraybackslash}m{0.42cm} 
        }
        \includegraphics[width=\linewidth]{images/more_results/seq1_3.5.png}
            &\includegraphics[width=\linewidth]{images/more_results/gt_rela_depth_3_3.558.png}
            &\includegraphics[width=\linewidth]{images/more_results/LMDD_rela_depth_3_3.558.png}
            &\includegraphics[width=\linewidth]{images/more_results/EMVS_rela_depth_3_3.558.png}
            &\includegraphics[width=\linewidth]{images/more_results/our_rela_depth_3_3.558.png}
            &\includegraphics[width=\linewidth]{images/more_results/colorbar_3_3.558.png}
		\\
        \includegraphics[width=\linewidth]{images/more_results/seq1_5.5.png}
            &\includegraphics[width=\linewidth]{images/more_results/gt_rela_depth_5_5.558.png}
            &\includegraphics[width=\linewidth]{images/more_results/LMDD_rela_depth_5_5.558.png}
            &\includegraphics[width=\linewidth]{images/more_results/EMVS_rela_depth_5_5.558.png}
            &\includegraphics[width=\linewidth]{images/more_results/our_rela_depth_5_5.558.png}
            &\includegraphics[width=\linewidth]{images/more_results/colorbar_5_5.558.png}
		\\
        \includegraphics[width=\linewidth]{images/more_results/seq1_11.5.png}
            &\includegraphics[width=\linewidth]{images/more_results/gt_rela_depth_11_11.550.png}
            &\includegraphics[width=\linewidth]{images/more_results/LMDD_rela_depth_11_11.550.png}
            &\includegraphics[width=\linewidth]{images/more_results/EMVS_rela_depth_11_11.550.png}
            &\includegraphics[width=\linewidth]{images/more_results/our_rela_depth_11_11.550.png}
            &\includegraphics[width=\linewidth]{images/more_results/colorbar_11_11.550.png}
		\\
        \includegraphics[width=\linewidth]{images/more_results/seq1_12.5.png}
            &\includegraphics[width=\linewidth]{images/more_results/gt_rela_depth_12_12.550.png}
            &\includegraphics[width=\linewidth]{images/more_results/LMDD_rela_depth_12_12.550.png}
            &\includegraphics[width=\linewidth]{images/more_results/EMVS_rela_depth_12_12.550.png}
            &\includegraphics[width=\linewidth]{images/more_results/our_rela_depth_12_12.550.png}
            &\includegraphics[width=\linewidth]{images/more_results/colorbar_12_12.550.png}
		\\
	\end{tabular}
	}
    \vspace{-1ex}
    \caption{EPBA results on synthetic data. 
    Panoramic maps have $2048 \times 1024$ px. 
    Initial camera rotations are obtained %by integrating the angular velocities estimated 
    using 
    % \gred{I think we need some color. It's too grayscale.
    % Could we plot some error maps, akin the trace map in this
    % % https://github.com/uzh-rpg/rpg_image_reconstruction_from_events/blob/master/data/synth1/sample_output/covariance_trace_colored_log_scale.jpg
    \label{fig:synth_refine}
    }
\end{figure*}

==> figures/objsize.tex <==
\begin{figure}%{0.4\textwidth}
  \begin{center}
    \includegraphics[width=0.65\linewidth]{images/n_m_f_20.png}
  \end{center}
  \caption{Evaluation of objects at different distance: foreground, middle ground and background.}
  \label{images:objsize}
  % \vspace{-0.5cm}
\end{figure}
